On the Importance of Exploration for Generalization in Reinforcement Learning

Existing approaches for improving generalization in deep reinforcement learning (RL) have mostly focused on representation learning, neglecting RL-specific aspects such as exploration. We hypothesize that the agent's exploration strategy plays a key role in its ability to generalize to new environments. Through a series of experiments in a tabular contextual MDP, we show that exploration is helpful not only for efficiently finding the optimal policy for the training environments but also for acquiring knowledge that helps decision making in unseen environments. Based on these observations, we propose EDE: Exploration via Distributional Ensemble, a method that encourages exploration of states with high epistemic uncertainty through an ensemble of Q-value distributions. Our algorithm is the first value-based approach to achieve state-of-the-art on both Procgen and Crafter, two benchmarks for generalization in RL with high-dimensional observations. The open-sourced implementation can be found at https://github.com/facebookresearch/ede .

==> neurips2023_ede_arxiv_arXiv/math.tex <==
\usepackage{amsmath,amsfonts,bm,bbm,amsthm, amssymb}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}


\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\mathbbm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}
\newcommand{\inner}[2]{\langle #1, #2 \rangle}
\newcommand{\norm}[1]{\left\|#1\right\|}

\newcommand{\parents}{Pa} %

\newcommand{\IN}{\text{in}}
\newcommand{\OUT}{\text{out}}
\newcommand{\conv}{\text{conv}}
\newcommand{\pad}{\text{pad}}
\newcommand{\pool}{\text{pool}}
\newcommand{\patch}{\text{patch}}
\newcommand{\nc}{\kappa}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\let\ab\allowbreak



\newcommand*{\horzbar}{\rule[0.5ex]{2.5ex}{0.3pt}}



\renewcommand{\mathbf}{\boldsymbol}
\newcommand{\mb}{\mathbf}
\newcommand{\mc}{\mathcal}
\newcommand{\mf}{\mathfrak}
\newcommand{\md}{\mathds}
\newcommand{\bb}{\mathbb}
\newcommand{\msf}{\mathsf}
\newcommand{\magnitude}[1]{ \left| #1 \right| }
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\condset}[2]{ \left\{ #1 \;\middle|\; #2 \right\} }


\newcommand{\reals}{\bb R}
\newcommand{\proj}{\mathrm{proj}}
\newcommand{\Cp}{\bb C}
\newcommand{\Z}{\bb Z}
\newcommand{\N}{\bb N}
\newcommand{\Sp}{\bb S}
\newcommand{\Ba}{\bb B}
\newcommand{\indicator}[1]{\mathbbm 1\{#1\}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\rvline}{\hspace*{-\arraycolsep}\vline\hspace*{-\arraycolsep}}
\makeatletter
\def\Ddots{\mathinner{\mkern1mu\raise\p@
\vbox{\kern7\p@\hbox{.}}\mkern2mu
\raise4\p@\hbox{.}\mkern2mu\raise7\p@\hbox{.}\mkern1mu}}
\makeatother


==> neurips2023_ede_arxiv_arXiv/sec_background.tex <==
\section{Background}

\textbf{Episodic Reinforcement Learning.} A \textit{Markov decision process} (MDP) is defined by the tuple $\gM = \big( \gS, \gA, R, P, \gamma, \mu \big)$, where $\gS$ is the state space, $\gA$ is the action space, $R: \gS \times \gA \rightarrow [R_{\min}, R_{\max} ]$ is the reward function
, $P: \gS \times \gA \times \gS \rightarrow \sR_{\geq 0}$ is the transition distribution, $\gamma \in (0, 1]$ is the discount factor, and $\mu: \gS \rightarrow \sR_{\geq 0}$ is the initial state distribution. We further denote the trajectory of an episode to be the sequence $\tau = (\vs_0, \va_0, r_0, \dots, \vs_T, \va_T, r_T, \vs_{T+1})$ where $r_t = R(\vs_t, \va_t)$ and $T$ is the length of the trajectory which can be infinite. 
If a trajectory is generated by a probabilistic policy $\pi: \gS \times \gA \rightarrow \sR_{\geq 0}$, $Z^\pi = \sum_{t=0}^T \gamma^t r_t$ is a random variable that describes the \textit{discounted return} the policy achieves. The objective is to find a $\pi^\star$ that maximizes the expected discounted return,
$\pi^\star = \argmax_\pi \E_{\tau \sim p^\pi(\cdot)}\left[ Z^\pi\right], \,\, \text{where} \,\, p^\pi(\tau) = \mu(\vs_0) \prod_{t=0}^T P(\vs_{t+1} \mid \vs_{t}, \va_{t}) \pi(\vs_{t}\mid \va_{t}).$
For simplicity, we will use $\E_{\pi}$ instead of $\E_{\tau \sim p^\pi(\cdot)}$ to denote the expectation over trajectories sampled from the policy $\pi$. With a slight abuse of notation, we use $Z^\pi(\vs, \va)$ to denote the conditional discounted return when starting at $\vs$ and taking action $\va$ (\ie{} $\vs_0 = \vs$ and $\va_0=\va$). Finally, without loss of generality, we assume all measures are discrete and their values lie within $[0, 1]$.

\textbf{Value-based methods}~\citep{watkins1992q} rely on a fundamental quantity in RL, the state-action value function, also referred to as the \textit{Q-function}, $Q^\pi(\vs, \va) = \E_{\pi}\left[Z^\pi \mid 
 \vs_0 = \vs, \,\,\va_0=\va\right]$.
The Q-function of a policy can be found at the fixed point of the Bellman operator, $\gT^\pi$~\citep{bellman1957markovian}, $\gT^\pi Q(\vs, \va) = \E_{  \vs'\sim P(\cdot \mid \vs, \va), \,\va' \sim \pi(\cdot\mid \vs')}\left[R(\vs, \va) + \gamma Q(\vs', \va') \right]$. \yi{The \emph{value function} for a state $\vs$ is defined as $V^\pi(\vs) = \E_{\va \sim \pi(\cdot \mid \vs)}[Q^\pi(\vs, \va)]$}.
\citet{bellemare2017distributional} extends the procedure to the distribution of discounted returns, $\gT^\pi Z(\vs, \va) \stackrel{d}{=} R(\vs, \va) + \gamma Z(\vs', \va'), \quad \vs' \sim P(\cdot \mid \vs, \va)\,\,\text{and}\,\,\va' \sim \pi(\cdot\mid \vs'),$
where $\stackrel{d}{=}$ denotes that two random variables have the same distributions. This extension is referred to as \textit{distributional RL} (we provide a more detailed description of QR-DQN, the distributional RL algorithm we use, in Appendix~\ref{app:qrdqn}). For value-based methods, the greedy policy is directly derived from the Q-function as $\pi(\va \mid \vs) = \mathbbm{1}_{\argmax_{\va'} Q(\va', \vs)}(\va)$.


\textbf{Generalization in Contextual MDPs.} A \textit{contextual Markov decision process} (CMDP)~\citep{hallak2015contextual} is a special class of \textit{partially observable Markov decision process} (POMDP) consisting of different MDPs, that share state and action spaces but have different $R$, $P$, and $\mu$. In addition to the standard assumptions of a CMDP, we assume the existence of a structured distribution $q_\gM$ over the MDPs. During training, we are given a (finite or infinite) number of training MDPs, $\Tilde{\gM}_{\text{train}} = \{\gM_1, \gM_2, \dots, \gM_n\}$, drawn from $q_\gM$ (\citet{ghosh2021generalization} refers to this setting as epistemic POMDP). We use $p^{\pi,\gM}(\tau)$ to denote the trajectory distribution of rolling out $\pi$ in $\gM$. The objective is to find a single policy $\pi$ that maximizes the expected discounted return over the entire distribution of MDPs, $\E_{\tau \sim p^{\pi, \gM}(\cdot), \gM \sim q_\gM(\cdot)}\left[ \sum_{t=0}^T \gamma^t r_t \right]$. \yi{We will refer to this quantity as the \textit{test return}\footnote{\yi{It may be useful to contrast this with the notion of generalization gap, the difference between training and test returns. Without good training performance, the generalization gap is not a meaningful measure: a random policy would have no generalization gap at all.}}. Since in RL the algorithm collects its own data, the appropriate notion of generalization is the performance a learning algorithm can achieve given a finite number of interactions. Crucially, if algorithm 1 achieves a better test return than algorithm 2 given the same number of interactions with $\gM_\text{train}$, we can say that algorithm 1 generalizes better than algorithm 2.} Furthermore, we assume the existence of $\pi^\star$ (potentially more than one) that is optimal for all $\gM \in \text{supp}(q_\gM)$, since otherwise, zero-shot generalization can be intractable~\citep{malik2021generalizable}. If the number of training environments is infinite, the challenge is learning good policies for all of them in a sample-efficient manner, \ie{} optimization; if it is finite, the challenge is also generalization to unseen environments. 


==> neurips2023_ede_arxiv_arXiv/sec_didactic.tex <==
\section{Generalization in a Tabular CMDP}
\label{sec:tabular}



Much of the literature treats generalization in deep RL as a pure representation learning problem~\citep{Song2020ObservationalOI, zhang2020invariant, zhang2020learning, Agarwal2021ContrastiveBS} and aims to improve it by using regularization~\citep{Farebrother2018GeneralizationAR, Zhang2018ADO, cobbe2018quantifying, igl2019generalization} or data augmentation~\citep{cobbe2018quantifying, lee2020network, ye2020rotation, kostrikov2020image, laskin2020reinforcement, Raileanu2020AutomaticDA, Wang2020ImprovingGI}. In this section, we will first show that the problem of generalization in RL extends \textbf{beyond representation learning} by considering a tabular CMDP, which does not require any representation learning. The goal is to provide intuition on the role of exploration for generalization in RL using a toy example. More specifically, we show that exploring the training environments can be helpful not only for finding rewards in those environments but also for making good decisions in new environments encountered at test time. 

Concretely, we consider a generic $5 \times 5$ grid environment (Figure~\ref{fig:reward}). During training, the agent always starts at a fixed initial state, $(x=0, \, y=0)$, and can move in $4$ cardinal directions (\ie{} up, down, left, right). The transition function is deterministic and if the agent moves against the boundary, it ends up at the same location. If the agent reaches the terminal state, $(x=4, \, y=0)$, it receives a large positive reward, $r=2$ and the episode ends. Otherwise, the agent receives a small negative reward, $r=-0.04$. At test time, the agent starts at a \textit{different} location, $(x=0, \, y=4)$. In other words, the train and test MDPs only differ by their initial state distribution. In addition, each episode is terminated at 250 steps (10 times the size of the state space) to speed up the simulation, but most episodes reach the terminal state before forced termination.

We study two classes of algorithms with different exploration strategies: (1) Q-learning with $\varepsilon$-greedy (\texttt{Greedy},~\citet{watkins1992q}), (2) Q-learning with UCB (\texttt{UCB},~\citet{auer2002finite}). To avoid any confounding effects of function approximation, we use \textit{tabular} policy parameterization for Q-values. Both \texttt{Greedy} and \texttt{UCB} use the same base Q-learning algorithm~\citep{watkins1992q}. \texttt{Greedy} explores with $\varepsilon$-greedy strategy which takes a random action with probability $\varepsilon$ and the best action according to the Q-function $\argmax_a Q(s,a)$ with probability $1 - \varepsilon$. In contrast, \texttt{UCB} is uncertainty-driven so it explores according to $\pi(a\mid s) = \mathbbm{1}(a=\argmax_{a'} Q(s,a') + c \sqrt{\log(t)/{N(s,a')}}),$ where $t$ is the total number of timesteps, $c$ is the exploration coefficient, and $N(s,a)$ is the number of times the agent has taken action $a$ in state $s$, with ties broken randomly\footnote{This \texttt{UCB} is a simple extension of the widely used bandits algorithm to MDP and does not enjoy the same regret guarantee, but we find it to be effective for the didactic purpose. \citet{azar2017minimax} presents a formal but much more complicated extension of the UCB algorithm for value iteration on MDPs. The \texttt{UCB} used is more similar to a count-based exploration bonus.}. While \texttt{Greedy} is a naive but widely used exploration strategy~\citep{sutton&barto}, \texttt{UCB} is an effective algorithm designed for multi-armed bandits~\citep{auer2002finite, audibert2009exploration}. \citet{chen2017ucb} showed that uncertainty-based exploration bonus also performs well in challenging RL environments. 
See Appendix~\ref{app:grid} for more details about the experimental setup.

\begin{figure*}[t]
     \centering
    \begin{subfigure}[b]{0.23\textwidth}
         \centering
        \includegraphics[width=\textwidth]{plots/reward.pdf}
        \caption{Tabular CMDP}
        \label{fig:reward}
    \end{subfigure}
    \begin{subfigure}[b]{0.26\textwidth}
         \centering
        \includegraphics[width=\textwidth]{plots/qlearning_egreedy.pdf}
        \caption{$\varepsilon$-greedy}
        \label{fig:ql-egreedy}
    \end{subfigure}
    \begin{subfigure}[b]{0.26\textwidth}
         \centering
        \includegraphics[width=\textwidth]{plots/qlearning_ucb.pdf}
        \caption{UCB}
        \label{fig:ql-ucb}
    \end{subfigure}
    \caption{(a) A tabular CMDP that illustrates the importance of exploration for generalization in RL. During training, the agent starts in the blue square, while at test time it starts in the orange square. In both cases, the goal is to get to the green square. The other plots show the mean and standard deviation of the train and test suboptimality (difference between optimal return and achieved return) over 100 runs for (b) Q-learning with $\varepsilon$-greedy exploration, (c) Q-learning with UCB exploration.}
    \label{fig:tabular-curves}
\end{figure*}



Each method's exploration strategy is controlled by a single hyperparamter. For each hyperparameter, we search over 10 values and run every value for 100 trials. Each trial lasts for 1000 episodes. The results (mean and standard deviation) of hyperparameters with the highest average test returns for each method are shown in Figures~\ref{fig:ql-egreedy} and~\ref{fig:ql-ucb}. We measure the performance of each method by its \textit{suboptimality}, \ie{} the difference between the undiscounted return achieved by the learned policy and the undiscounted return of the optimal policy. While all three methods are able to quickly achieve an optimal return for the training MDP, their performances on the test MDP differ drastically. First, we observe that \texttt{Greedy} has the worst generalization performance and the highest variance. On the other hand, \texttt{UCB} can reliably find the optimal policy for the test MDP as the final return has a negligible variance. In Appendix~\ref{app:dynamic}, we provide another set of simulations based on \textit{changing dynamics} and make similar observations. These experiments show that \textbf{more effective exploration of the training environments can result in better generalization to new environments}.



It is natural to ask whether this example is relevant for realistic deep RL problems. \yi{
Analytically, we can motivate the importance of exploration for generalization using \emph{sub-MDPs}~\citep{kearns1998finite} and the \emph{sample complexity} of Q-learning~\citep{li2020sample}. Due to space constraints, we develop this argument in Appendix~\ref{app:theory}.} \yi{Conceptually,} the tabular CMDP with two initial state distributions captures a common phenomenon in more challenging CMDPs like Procgen, namely that at test time, the agent can often end up in \yi{suboptimal} 
states that are \yi{rarely visited by simple exploration on} the training MDPs. Having explored such states during training can help the agent recover from suboptimal states at test time. See Figure~\ref{fig:simple_bifgish_main} and Appendix~\ref{app:scenario} for an illustrative example inspired by one of the Procgen games. This is similar to covariate shift in imitation learning where the agent's suboptimality can compound over time. The effect of efficient exploration is, in spirit, similar to that of DAgger~\citep{ross2011reduction} --- it helps the agent learn how to recover from situations that are rare during training. 


\yi{In Appendix~\ref{app:alternative}, we explore some other interpretations for why exploration improves generalization (which are also related to the sample complexity of Q-learning). In addition, we also explore other potential reasons for why current RL methods generalize poorly in Appendix~\ref{app:poorgen}. Note that we do not claim exploration to be the only way of improving generalization in RL. In Appendix~\ref{app:pg} and~\ref{app:sarsa}, we study other potential avenues for improving generalization. The benefits of exploration are complementary to these approaches, and they may be combined to further improve performance. In this paper, we focus on using exploration to improve generalization in contextual MDPs.}

\begin{figure}[t]
     \centering
    \begin{subfigure}[b]{0.8\textwidth}
         \centering
        \includegraphics[width=\textwidth]{plots/simple_bigfish.png}
    \end{subfigure}
    \caption{\yi{A simplified version of \texttt{bigfish} in Procgen (Figure~\ref{fig:bigfish}) that captures the spirit of the grid world example from Figure~\ref{fig:reward}. The green dot represents the agent and the red dots represent the enemies (see Appendix~\ref{app:scenario} for more details). The goal is to eat smaller dots while avoiding larger dots. An agent that explores both trajectories in the training MDP could recover the optimal behavior on the test MDP whereas an agent that only focuses on solving the training MDP would fail.}}
    \vspace{-3mm}
    \label{fig:simple_bifgish_main}
\end{figure}

















==> neurips2023_ede_arxiv_arXiv/sec_experiment.tex <==

\begin{figure*}[t]
     \centering
    \begin{subfigure}[b]{1.0\textwidth}
         \centering
        \includegraphics[width=\textwidth]{plots/main_comparison.pdf}
    \end{subfigure}
    \caption{Test performance of different methods on the Procgen benchmark across 5 runs. Our method greatly outperforms all baselines in terms of median and IQM (the more statistically robust metrics) and is competitive with the state-of-the-art policy optimization methods in terms of mean and optimality gap. The optimality gap is equal to 1-mean for the evaluation configuration we chose.}
        \label{fig:final}
        \vspace{-2mm}
\end{figure*}

\section{Experiments}



\subsection{Procgen} 
We compare our method with 3 representative baselines on the standard Procgen benchmark (\ie{} 25M steps and easy mode) as suggested by \citet{cobbe2018quantifying}: (1) \texttt{QR-DQN} which is the prior state-of-the-art value-based method on Procgen~\citep{ehrenberg2022study};
(2) \texttt{PPO} which is a popular policy optimization baseline on which most competitive methods are built; and (3) \texttt{IDAAC} which is state-of-the-art on Procgen and is built on \texttt{PPO}. We tune all hyperparameters of our method on the game \texttt{bigfish} only and evaluate all algorithms using the 4 metrics proposed in~\citet{agarwal2021deep}. We run each algorithm on every game for 5 seeds and report the aggregated min-max normalized scores on the full test distribution, and the estimated bootstrap-estimated 95\% confidence interval in Figure~\ref{fig:final} (simulated with the runs). Our approach significantly outperforms the other baselines in terms of median and interquartile mean (IQM) (which are the more statistically robust metrics according to~\citet{agarwal2021deep}). In particular, it achieves almost 3 times the median score of \texttt{QR-DQN} and more than 2 times the IQM of \texttt{QR-DQN}. In terms of mean and optimality gap, our method is competitive with \texttt{IDAAC} and outperforms all the other baselines. To the best of our knowledge, this is the first value-based method that achieves such strong performance on Procgen. See Appendices~\ref{app:hps},~\ref{app:all_algo}, and~\ref{app:sensitivity} for more details about our experiments, results, and hyperparameters.




\textbf{Ablations and Exploration Baselines.} We aim to better understand how each component of our algorithm contributes to the final performance by running a number of ablations. 
In addition, we compare with other popular exploration techniques for value-based algorithms. Since many of the existing approaches are designed for \textsc{DQN}, we also adapt a subset of them to \textsc{QR-DQN} for a complete comparison. The points of comparison we use are: (1) Bootstrapped DQN~\citep{osband2015bootstrapped} which uses bootstrapping to train several copies of models that have distinct exploration behaviors, (2) UCB~\citep{chen2017ucb} which uses an ensemble of models to do uncertainty estimation, (3) $\epsilon z$-greedy exploration~\citep{dabney2021temporallyextended} which repeats the same random action (following a zeta distribution) to achieve temporally extended exploration, (4) UA-DQN~\citep{clements2019estimating}, and (5) NoisyNet~\citep{fortunato2017noisy} which adds trainable noise to the linear layers~\footnote{\citet{Taiga2020On} found that, on the whole Atari suite, NoisyNet outperforms more specialized exploration strategies such as ICM~\citep{pathak2017curiosity} and RND~\citep{burda2018exploration}. This suggests that these exploration methods may have overfitted to sparse reward environments.}. When UCB is combined with QR-DQN, we use the epistemic uncertainty unless specified otherwise. The results are shown in Figure~\ref{fig:ablation}. Details can be found in Appendix~\ref{app:hps}.

First, note that both using the epistemic uncertainty via UCB and training on diverse data from TEE are crucial for the strong performance of \ours{}, with QR-DQN+TEE being worse than QR-DQN+UCB which is itself worse than \ours{}. Without epistemic uncertainty, the agent cannot do very well even if it trains on diverse data, \ie{} \ours{} is better than QR-DQN+TEE. Similarly, even if the agent uses epistemic uncertainty, it can still further improve its performance by training on diverse data, \ie{} \ours{} is better than QR-DQN+UCB.

Both Bootstrapped DQN and DQN+UCB, which minimize the total uncertainty rather than only the epistemic one, perform worse than DQN, although both are competitive exploration methods on Atari. This highlights the importance of using distributional RL in CMDPs in order to measure epistemic uncertainty. QR-DQN+UCB on the other hand outperforms QR-DQN and DQN because it only targets the epistemic uncertainty. In Figure~\ref{fig:uncertainty} from Appendix~\ref{app:analysis}, we show that indeed exploring with the total uncertainty $\sigma^2$ performs significantly worse at test time than exploring with only the epistemic uncertainty $\sigma_\text{epi}^2$. UA-DQN also performs worse than QR-DQN+UCB suggesting that deep ensemble may have better uncertainty estimation (Appendix~\ref{app:uncert-analysis}).

QR-DQN with $\epsilon z$-greedy exploration marginally improves upon the base QR-DQN, but remains significantly worse than \ours{}. This may be due to the fact that $\epsilon z$-greedy exploration can induce temporally extended exploration but it is not aware of the agent's uncertainty. 
Not accounting for uncertainty can be detrimental since CMDPs can have a much larger number of effective states than singleton MDPs. If the models have gathered enough information about a state, further exploring that state can hurt sample efficiency, regardless of whether the exploration is temporally extended.

NoisyNet performs better than the other points of comparison we consider \yi{but it is still} worse than \ours{}. The exploration behaviors of NoisyNet are naturally adaptive --- the agents will take into account what they have already learned. While a direct theoretical comparison between NoisyNet and our method is hard to establish, we believe adaptivity is a common thread for methods that perform well on CMDPs.
Nonetheless, if we consider IQM, none of these methods significantly outperforms one another whereas our method achieves a much higher IQM. Note that TEE cannot be easily applied to NoisyNets and $\epsilon z$-greedy which implicitly use an schedule.



\begin{figure*}[t]
     \centering
    \begin{subfigure}[b]{1.0\textwidth}
         \centering
        \includegraphics[width=\textwidth]{plots/ablation.pdf}
    \end{subfigure}
    \caption{Test performance of different exploration methods on the Procgen benchmark across 5 runs. 
    }
    \label{fig:ablation}
\end{figure*}

\subsection{Crafter}





\begin{wraptable}[11]{r}{0.3\textwidth}
    \centering
    \small
    \vspace{-5mm}
    \caption{Results on Crafter after 1M steps and over 10 runs.}
        \vspace{3mm}
    \begin{tabular}{lr}
    \toprule
    \textbf{Method} & \textbf{Score (\%)}  \\
    \midrule
    \ours{} (ours) & $11.7\pm1.0$  \\
    \midrule
    Rainbow& $4.3\pm0.2 $   \\
    PPO& $4.6\pm0.3 $     \\
    DreamerV2 & $10.0\pm1.2 $    \\
    LSTM-SPCNN & $12.1 \pm 0.8$\\
    \bottomrule
    \end{tabular}

    \label{tab:crafter}
\end{wraptable}
To test the generality of our method beyond the Procgen benchmark, we conduct experiments on the Crafter environment~\citep{hafner2022benchmarking}. Making progress on Crafter requires a wide range of capabilities such as strong generalization, deep exploration, and long-term reasoning. Crafter evaluates agents using a score that summarizes the agent's abilities into a single number. Each episode is procedurally generated, so the number of training environments is practically infinite. While Crafter does not test generalization to new environments, it still requires generalization across the training environments in order to efficiently train on all of them. We build our method on top of the Rainbow implementation~\citep{hessel2018rainbow} provided in the open-sourced code of~\citet{hafner2022benchmarking} \yi{and \emph{only} changed the exploration to use \ours{}.}



We use Thompson sampling instead of UCB+TEE since only one environment is used. As seen in Table~\ref{tab:crafter}, our algorithm achieves significantly higher scores
compared to all the baselines presented in \citet{hafner2022benchmarking}, including DreamerV2~\citep{hafner2021mastering} which is a state-of-the-art model-based RL algorithm. \yi{It is also competitive with LSTM-SPCNN~\citep{stanic2022an} which uses a specialized architecture with two orders of magnitude more parameters and extensive hyperparameter tuning.} The significant improvement over Rainbow, which is a competitive value-based approach, suggests that the exploration strategy is crucial for improving performance on such CMDPs. 





==> neurips2023_ede_arxiv_arXiv/sec_method.tex <==
\section{Exploration via Distributional Ensemble}

In the previous section, we showed we can improve generalization via exploration in the tabular setting. In this section, we would like to extend this idea to deep RL with function approximation. While in the tabular setting shown above there is no intrinsic stochasticity, environments can in general be stochastic (\eg{} random transitions, or random unobserved contexts). At a high level, epistemic uncertainty reflects a lack of knowledge which can be addressed by collecting more data, while aleatoric uncertainty reflects the intrinsic noise in the data which cannot be reduced regardless of how much data is collected. One goal of exploration is to gather information about states with high epistemic uncertainty~\citep{o2018uncertainty} since aleatoric uncertainty cannot be reduced, but typical estimates can contain both types of uncertainties~\citep{kendall2017uncertainties}. In CMDPs, this is particularly important because a large source of aleatoric uncertainty is not knowing which context the agent is in~\citep{raileanu2021decoupling}.

\yi{
In this section, we introduce \emph{Exploration via Distributional Ensemble} (\ours{}), a method that encourages the exploration of states with high epistemic uncertainty. Our method builds on several important ideas from prior works, the most important of which are deep ensembles and distributional RL. While ensembles are a useful way of measuring uncertainty in neural networks~\citep{lakshminarayanan2017simple}, such estimates typically contain both epistemic and aleatoric uncertainty. To address this problem, we build on \citet{clements2019estimating} which introduced an approach for disentangling the epistemic uncertainty from the aleatoric uncertainty of the learned Q-values. 
}

\textbf{Uncertainty Estimation.} \citet{clements2019estimating} showed that learning the quantiles for QR-DQN~\citep{dabney2018distributional} can be formulated as a Bayesian inference problem, given access to a posterior $p(\vtheta \mid \gD)$, where $\vtheta$ is the discretized quantiles of $Z(\vs, \va)$, and $\gD$ is the dataset of experience on which the quantiles are estimated. Let $j \in [N]$ denote the index for the $j^\text{th}$ quantile and $\gU\{1, N\}$ denote the uniform distribution over integers between $1$ and $N$. The uncertainty of the Q-value, $Q(\vs, \va) = \E_{j \sim \gU\{1, N\}}\left[ \vtheta_j(\vs, \va)\right]$, is the relevant quantity that can inform exploration. The overall uncertainty $\sigma^2 = \Var_{\vtheta \sim p(\vtheta \mid \gD)}\left[Q(\vs, \va)\right]$ can be decomposed into \textit{epistemic uncertainty} $\sigma^2_\text{epi}(\vs, \va)$ and \textit{aleatoric uncertainty} $\sigma^2_\text{ale}(\vs, \va)$ such that $\sigma^2(\vs, \va) =\sigma^2_\text{epi}(\vs, \va) + \sigma^2_\text{ale}(\vs, \va)$, where,

\begin{small}
\begin{align}
    \sigma^2_\text{epi}(\vs, \va) = \E_{j \sim \gU\{1, N\}}\left[\Var_{\vtheta \sim p(\vtheta \mid \gD)}\left[\vtheta_{j}(\vs, \va) \right]\right], \,
    \sigma^2_\text{ale}(\vs, \va) = \Var_{j \sim \gU\{1, N\}}\left[\E_{\vtheta \sim p(\vtheta \mid \gD)}\left[\vtheta_{j}(\vs, \va) \right]\right].
\end{align}
\end{small}%

Ideally, given an infinite or sufficiently large amount of diverse experience, one would expect the posterior to concentrate on the true quantile $\vtheta^\star$, so $\Var_{\vtheta \sim p(\vtheta \mid \gD)}\left[\vtheta_{j}(\vs, \va) \right]$ and consequently $\sigma^2_\text{epi}(\vs, \va)=0$. $\sigma^2_\text{ale}$ would be non-zero if the true quantiles have different values. Intuitively, to improve the sample efficiency, the agent should visit state-action pairs with high epistemic uncertainty in order to learn more about the environment~\citep{chen2017ucb}. It should be noted that the majority of the literature on uncertainty estimation focuses on supervised learning; in RL, due to various factors such as bootstrapping, non-stationarity, limited model capacity, and approximate sampling, the uncertainty estimation generally contains errors but empirically even biased epistemic uncertainty is beneficial for exploration. 
We refer interested readers to \citet{charpentier2022disentangling} for a more thorough discussion.

Sampling from $p(\vtheta \mid \gD)$ is computationally intractable for complex MDPs and function approximators such as neural networks.
\citet{clements2019estimating} approximates samples from $p(\vtheta \mid \gD)$ with randomized MAP
sampling~\citep{pearce2020uncertainty} which assumes a Gaussian prior over the model parameters. However, the unimodal nature of a Gaussian in parameter space may not have enough diversity for effective uncertainty estimation. Many works have demonstrated that \textit{deep ensembles} tend to outperform other approximate posterior sampling techniques~\citep{lakshminarayanan2017simple, fort2019deep} in supervised learning. Motivated by these observations, we propose to maintain $M$ copies of fully-connected value heads, $g_i: \sR^{d} \rightarrow \sR^{|\gA| \times N}$ that share a single feature extractor $f: \gS \rightarrow \sR^{d}$, similar to \citet{osband2016deep}. However, we train each value head with \textit{different} mini-batches and random initialization (\ie{} deep ensemble) instead of distinct data subsets (\ie{} bootstrapping). This is consistent with \citet{lee2021sunrise} which shows deep ensembles usually perform better than bootstrapping for estimating the uncertainty of Q-values but, unlike \ours{}, they do not decompose uncertainties. 

 Concretely, $i \in [M]$ is the index for $M$ ensemble heads of the Q-network, and $j \in [N]$ is the index of the quantiles. The output of the $i^\text{th}$ head for state $\vs$ and action $\va$ is $\vtheta_i(\vs, \va) \in \sR^{N}$, where the $j^\text{th}$ coordinate, and $\vtheta_{ij}(\vs, \va)$ is the $j^\text{th}$ quantile of the predicted state-action value distribution for that head. The finite sample estimates of the two uncertainties are:
\begin{small}
\begin{align}
    \hat{\sigma}^2_\text{epi}(\vs, \va) = \frac{1}{N\cdot M}\sum_{j=1}^N\sum_{i=1}^M\left(\vtheta_{ij}(\vs, \va) - \Bar{\vtheta}_j(\vs, \va)\right)^2, \,
    \hat{\sigma}^2_\text{ale}(\vs, \va) = \frac{1}{N} \sum_{j=1}^N \left(\Bar{\vtheta}_j(\vs, \va) - Q(\vs, \va)\right)^2, 
    \label{eq:uncertainty}
\end{align}
\end{small}%
where $\Bar{\vtheta}_j(\vs, \va) = \frac{1}{M}\sum_{i=1}^{M} \vtheta_{ij}(\vs, \va)$ and $Q(\vs, \va) = \frac{1}{N}\sum_{j=1}^{N}\Bar{\vtheta}_j(\vs, \va).$

\textbf{Exploration Policy.} There are two natural ways to use this uncertainty. The first one is by using Thompson sampling~\citep{thompson1933likelihood} where the exploration policy is defined by sampling Q-values from the posterior:
\begin{align}
    \pi_\text{ts}(\va \mid \vs) = \mathbbm{1}_{\argmax_{\va'} \,\, \xi(\vs, \va')}\left(\va\right), \quad \text{where} \quad \xi(\vs, \va') \sim \gN\left(Q(\vs, \va'), \, \varphi \,\, \hat{\sigma}_\text{epi}(\vs, \va')\right).
    \label{eq:ts}
\end{align}
$\varphi \in \sR_{\geq 0}$ is a coefficient that controls how the agent balances exploration and exploitation. Alternatively, we can use the upper-confidence bound (UCB,~\citet{chen2017ucb}):
\begin{align}
    \pi_\text{ucb}(\va \mid \vs) = \mathbbm{1}_{\va^\star}\left(\va\right),\quad \text{where}\,\, \va^\star = \argmax_{\va'} \, Q(\vs, \va') + \varphi \,\, \hat{\sigma}_\text{epi}(\vs, \va'),
\end{align}
which we found to achieve better results in CMDPs than Thompson sampling \citep{clements2019estimating} on Procgen when we use multiple parallel workers to collect experience, especially when combined with the next technique.

\textbf{Equalized Exploration.} Due to function approximation, the model may lose knowledge of some parts of the state space if it does not see them often enough. 
Even with UCB, this can still happen after the agent learns a good policy on the training environments.
To increase the data diversity, we propose to use different exploration coefficients for each copy of the model used to collect experience. Concretely, we have $K$ actors with synchronized weights; the $k^\text{th}$ actor collects experience with the following policy:
\begin{align}
    \pi_\text{ucb}^{(k)}(\va \mid \vs) = \mathbbm{1}_{\va^\star}\left(\va\right),\quad
    \text{where}\,\,\va^\star = \argmax_{\va'} \, Q(\vs, \va') + \left(\varphi \, \lambda^{1 + \frac{k}{K-1} \alpha}\right) \hat{\sigma}_\text{epi}(\vs, \va').
    \label{eq:ucb}
\end{align}
$\lambda \in (0,1)$ and $\alpha \in \sR_{> 0}$ are hyperparameters that control the shape of the coefficient distribution. We will refer to this technique as \textit{temporally equalized exploration} (TEE). TEE is inspired by \citet{horgan2018distributed} which uses different values of $\varepsilon$ for the $\varepsilon$-greedy exploration for each actor. In practice, the performances are not sensitive to $\lambda$ and $\alpha$ (see Figure~\ref{fig:tee-hp} in Appendix~\ref{app:analysis}). Both learning and experience collection take place on a single machine and no prioritized experience replay~\citep{schaul2015prioritized} is used since prior work found it ineffective in CMDPs~\citep{ehrenberg2022study}. 

To summarize, our agent explores the environment in order to gather information about states with high epistemic uncertainty which is measured using ensembles and distributional RL. We build on the algorithm proposed in~\citet{clements2019estimating} for estimating the epistemic uncertainty, but we use deep ensemble instead of MAP~\citep{pearce2020uncertainty}, and use either UCB or Thompson sampling depending on the task and setting. In addition, for UCB, we propose that each actor uses a different exploration coefficient for more diverse data. While variations of the components of our algorithm have been used in prior works, this particular combination is new (see Appendix~\ref{app:algo}).
Our ablation experiments show that each design choice is important and \yi{\textbf{applying these techniques individually or na\"\i vely combining them performs significantly worse.}}



==> neurips2023_ede_arxiv_arXiv/sec_related_works.tex <==

\section{Related Works}
\textbf{Generalization in RL.} A large body of work has emphasized the challenges of training RL agents that can generalize to new environments and tasks~\citep{Rajeswaran2017TowardsGA, Machado2018RevisitingTA, Justesen2018IlluminatingGI, Packer2018AssessingGI, Zhang2018ADO, Zhang2018ASO, Nichol2018GottaLF, cobbe2018quantifying, cobbe2019leveraging, Juliani2019ObstacleTA, Kuttler2020TheNL, Grigsby2020MeasuringVG, Chen2020ReinforcementLG, Bengio2020InterferenceAG, Bertrn2020InstanceBG, ghosh2021generalization,kirk2021survey,
ajay2021understanding, ehrenberg2022study, lyle2022learning}. This form of generalization is different from generalization in singleton MDP which refers to function approximators generalizing to different states within the same MDP. A natural way to alleviate overfitting is to apply widely-used regularization techniques such as implicit regularization~\citep{Song2020ObservationalOI}, dropout~\citep{igl2019generalization}, batch normalization~\citep{Farebrother2018GeneralizationAR}, or data augmentation~\citep{ ye2020rotation, lee2020network, laskin2020reinforcement, Raileanu2020AutomaticDA, Wang2020ImprovingGI, yarats2021mastering, hansen2021generalization, hansen2021stabilizing, ko2022efficient}. Another family of methods aims to learn better state representations via bisimulation metrics~\citep{zhang2020learning, zhang2020invariant, Agarwal2021ContrastiveBS}, information bottlenecks~\citep{igl2019generalization, fan2022dribo}, attention mechanisms~\citep{carvalho2021feature}, contrastive learning~\citep{mazoure2021improving}, adversarial learning~\citep{roy2020visual, fu2021learning, rahman2021adversarial}, or decoupling representation learning from decision making~\citep{Stooke2020DecouplingRL, Sonar2020InvariantPO}.
Other approaches use information-theoretic approaches~\citep{Chen2020ReinforcementLG, Mazoure2020DeepRA}, non-stationarity reduction~\citep{Igl2020TheIO, nikishin2022primacy}, curriculum learning~\citep{Jiang2020PrioritizedLR, team2021open, jiang2021replay, parker2022evolving}, planning~\citep{anand2021procedural}, forward-backward representations~\citep{touati2021learning}, or diverse policies~\citep{kumar2020one}. More similar to our work, ~\citet{raileanu2021decoupling} show that the value function can overfit when trained on CMDPs and propose to decouple the policy from the value optimization to train more robust policies. However, this approach cannot be applied to value-based methods since the policy is directly defined by the Q-function. Most of the above works focus on policy optimization methods, and none emphasizes the key role exploration plays in training more general agents. In contrast, our goal is to understand why value-based methods are significantly worse on CMDPs. 


\textbf{Exploration.} Exploration is a fundamental aspect of RL~\citep{kolter2009near, fruit2017exploration, tarbouriech2020no}. Common approaches include $\varepsilon$-greedy~\citep{sutton&barto}, count-based exploration~\citep{strehl2008analysis, bellemare2016unifying, machado2020count}, curiosity-based exploration~\citep{schmidhuber1991possibility, CS, pathak2017curiosity}, or novelty-based methods specifically designed for exploring sparse reward CMDPs~\citep{RIDE, zha2021rank, AGAC, NovelD}. These methods are based on policy optimization and focus on training agents in sparse reward CMDPs. In contrast, we are interested in leveraging exploration as a way of improving the generalization of value-based methods to new MDPs (including dense reward ones). Some of the most popular methods for improving exploration in value-based algorithms use noise~\citep{osband2016generalization, fortunato2017noisy}, bootstrapping~\citep{osband2015bootstrapped, osband2016deep}, ensembles~\citep{chen2017ucb, lee2020network, liang2022reducing}, uncertainty estimation~\citep{osband2013more, o2018uncertainty, clements2019estimating}, or distributional RL~\citep{mavrin2019distributional}. The main goal of these works was to use exploration to improve sample efficiency on singleton MDPs that require temporally extended exploration. Another related area is task-agnostic RL~\citep{pong2019skew, zhang2020task} where the agent explores the environment without reward and tries to learn a down-stream task with reward, but to our knowledge, these methods have not been successfully adapted to standard benchmarks like Procgen. Our work is the first one to highlight the role of exploration for faster training on contextual MDPs and better generalization to unseen MDPs. Our work also builds on the distributional RL perspective~\citep{bellemare2017distributional}, which is useful in CMDPs for avoiding value overfitting~\citep{raileanu2021decoupling}.


==> neurips2023_ede_arxiv_arXiv/sec_theory.tex <==
\section{A Combinatorial Framework of Feature Learning}
\label{sec:toy_model}

In this section, we present a new framework of feature learning for a binary classification\footnote{This can be extended to multi-class without significant modification.} based on the insights from the experiments above. We saw in \hyperlink{obs1}{O.1} that the distribution of features is long-tailed. This means a relative small number of unique features constitute a large proportion of all the features that appear in the data. To facilitate analysis, we will assume there are two types of features, \textit{dominant features} and \textit{rare features}, where the dominant features appear with much higher probability than rare features. Further, we observed that data with high confidence tend to have much fewer features than the ones with high confidence (\hyperlink{obs2}{O.2}). To model this behavior, we will assume that there are two types of data points: \textit{dominant data} and \textit{rare data}. The former contains a small number of dominant features and the later contains a larger number of rare features. This is another simplification based on \hyperlink{obs2}{O.2}, which shows that high-confidence data tend to have fewer high-frequency features.

\paragraph{Definitions and additional notations.} Before describing the full model, we first define the parameters of the model as well as some additional notations:
\begin{itemize}
    \item $p_d$: the proportion of all data that are dominant.
    \item $p_r$: the proportion of all data that are rare. This parameter is equal to $1-p_d$.
    \item $c$: the total model capacity. It represents how many features a single model can learn.
     \item $t_d$: the total number of dominant features available in the data for one class.
    \item $t_r$: the total number of rare features available in the data for one class.
    \item $n_d$: the total number of dominant features a single dominant data point has. $n_d \leq t_d$.
    \item $n_r$: the total number of rare features a single rare data point has. $n_r \leq t_r$.
\end{itemize}
We will use $\Pi(\cdot)$ to denote the set of all features a model or a feature have.

\paragraph{Data generating process.} We can see the data generating process as the following sampling procedure. First, we decide which class the data point belongs to. We are considering a class balanced binary classification problem so each class occurs with equal probability of $\frac{1}{2}$. Then, we decide whether the data point is dominant or rare. This is the equivalent to sampling from a Bernoulli distribution, $\text{Ber}(p_d)$. If the data point is dominant, we sample $n_d$ dominant features uniformly \textit{without} replacement. Vice versa, if the data point is rare, we sample $n_r$ dominant features uniformly \textit{without} replacement. It is easy to verify that the proportion of dominant data points and features is $p_d$ and the proportion of rare data points and features is $p_r$.

\paragraph{How the models learn.} We saw in \hyperlink{obs3}{O.3} that the frequency of features occurring in different models is positively correlated with the frequency at which the features occur in the data. We can model the learning process as another \textit{sampling-without-replacement} process where the probability that a model learns a feature is \textit{proportional} to the frequency at which the feature occurs in the data. Under this assumption, in expectation, $c_d = \frac{1}{2} p_d  c$ of the features in a single model would be dominant features for a single class, and $c_r = \frac{1}{2} p_r  c$ of the features for a single class would be rare. We can further simplify this process by assuming that the model will always sample $c_d$ dominant features for each class, and $c_r$ rare features for each class\footnote{Both $c_r$ and $c_d$ are rounded to the nearest integer such that the total number of features in a model is still $c$.}.

\paragraph{How the models make predictions.} For a data point $x$ and a model $f$, we assume that the model will correctly classify $x$ if the overlap between the features of $x$ and the features of $f$ is not empty. Otherwise, the model will perform a random guess. The expected error that a single model $f$ makes on a single datum pair $(x,y)$ is thus $\msf{err}(f, x, y) = \frac{1}{2}\mathbbm{1}\left\{\Pi(f) \cap \Pi(x) = \varnothing \right\}$.
Further, given a pair of models $(f,g)$ and a single datum pair $(x,y)$, there are three distinct behaviors for how they will make predictions. \textbf{(1)} The two models will always agree with each other if both of them share feature with $x$, since both will classify $x$ correctly (i.e., if $|\Pi(f) \cap \Pi(x)| > 0$ and $|\Pi(g) \cap \Pi(x)| > 0$). \textbf{(2)} If the models both do not share any features with $x$, then by the previous assumptions, the models will make random guesses; however, if the models share features with each other, their random guesses will not be independent from each other (\hyperlink{obs4}{O.4}). We hypothesize that how two models agree with each other is a function of $k$, the number of features they share, and $c$, the model capacity. We capture this intuition with an \textit{agreement function},  $\zeta: \sN \times \sN \rightarrow [0, 1]$, which returns the probability that two models will agree based on how many features they share relative to the full model capacity. This function is crucial for understanding how models make mistakes. \textbf{(3)} Finally, if the models do not share any features with each other or with $x$, both models will perform independent random guesses, in which case they will agree $50\%$ of the time.

\paragraph{Remarks.} An important difference between this model and the multi-view model from~\citet{allen2020towards} is that our model does not treat all features as equal. Indeed, the experiments in Section~\ref{sec:exp} show that features demonstrate a wide range behaviors in terms of how often they occur in the data and how they interact with the models. Another notable difference is that in~\citet{allen2020towards}, the multi-view portion of the dataset -- which intuitively are easier to classify -- contains \textit{all} the features in the data. In reality, the ``easy'' part of the data that a large portion of the models classify correctly actually contain much fewer features. These observations suggest that having different types of features is perhaps a more accurate description of nature. Nonetheless, we do not describe the exact mechanism of how feature learning actually happens under our model since we are not assuming any particular hypothesis class. The spirit of our model of feature learning is close to that of~\citet{allen2020towards} and we believe a similar iterative analysis can be applied to our model.

It is also natural to question whether the simplification where a single feature is sufficient for determining the class is sensible. Indeed, in practice, a classifier likely uses more than one feature to determine the correct class. We believe that this simplification is realistic as we are considering a binary classification problem in this framework, and that allowing more features to participate in determining the true class makes the model more expressive but should not fundamentally alter the behavior of the system.
Further, the true distributions of features and data are evidently more complex --- dominant data can contain rare features, and, vice versa, rare data can also contain some dominant features. In fact, the dichotomy may no longer be appropriate as the distribution of features and data becomes more complicated --- both features and data can lie on a continuous spectrum between ``dominant'' and ``rare'' (Figure~\ref{fig:feat_freq} and \ref{fig:conf_feat}). These changes can be smoothly incorporated into the framework by modifying the distribution of features but doing so can increase the complexity of the analysis. An exact analytical solution may become unattainable, but we could leverage tail bounds to characterize the system, a promising direction for future works. Still, we will see that this relatively simplified model readily offers interesting insights into observed phenomena. 

\subsection{Analytical Forms of Accuracy and Agreement}
Using this model, the analytical form of expected accuracy, $\msf{Acc}$, and expected agreement rates, $\msf{Agr}$, can be derived through combinatorics.  All propositions are proven in Appendix~\ref{app:proof}, but the chief point here is that these are both computable in closed form.

\begin{proposition}
Under the model defined above, the expected accuracy over the model distribution and data distribution is:
\begin{align}\label{eqn:acc}
    \msf{Acc} = p_d\left( 1- \frac{1}{2}\frac{{t_d-c_d \choose n_d}}{{t_d \choose n_d}} \right) + p_r\left( 1- \frac{1}{2}\frac{{t_r-c_r \choose n_r}}{{t_r \choose n_r}} \right).
\end{align}
\end{proposition}

\begin{proposition}
For the model above, let ${n \choose r}=0$ when $n < 0$, $r < 0$ or $n < r$,
and let:
\begingroup
\allowdisplaybreaks
\begin{small}
\begin{align*}
    q_1 &= p_d \left(1-\frac{{t_h-c_d \choose n_d}}{{t_d \choose n_d}}\right)^2 + p_r \left(1-\frac{{t_r-c_r \choose n_r}}{{t_r \choose n_r}}\right)^2,   \\
    q_2(k) &= p_d \frac{{t_d-n_d \choose c_d}^2}{{t_d \choose c_d}^2} \left( \sum_{a+b=k} \frac{{c_d \choose a}{t_d-n_d-c_d \choose c_d - a}}{{t_d-n_d \choose c_d}} \frac{{c_r \choose b}{t_r-c_r \choose c_r - b}}{{t_r \choose c_r}} \right) \\
    & \,\,\,\, + p_r \frac{{t_r-n_r \choose c_r}^2}{{t_r \choose c_r}^2} \left( \sum_{a+b=k} \frac{{c_d \choose a}{t_d-c_d \choose c_d - a}}{{t_d \choose c_d}} \frac{{c_r \choose b}{t_r-n_r-c_r \choose c_r - b}}{{t_r-n_r \choose c_r}} \right),
\end{align*}
\end{small}
\endgroup
then the expected agreement between an i.i.d pair of models $(f,g)$ drawn for the model distribution is:
\begin{align}\label{eqn:agr}
    \msf{Agr} = \frac{1}{2} + \frac{1}{2}q_1 + \sum_{k=1}^c \left (\zeta(k, c) - \frac{1}{2} \right) q_2(k).
\end{align}

\end{proposition}

Further, we discuss the origin of irreducible \textit{generalization error} and other properties of this framework in Appendix~\ref{app:error} and show a potential connection between feature learning and data scaling~\citep{hestness2017deep}.

\subsection{Numerical Simulation}

\begin{figure*}[h]
     \centering
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/p_d.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/t_d.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/t_r.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/t_r_t_d.pdf}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/c.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/n_d.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/n_r.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/n_r_n_d.pdf}
    \end{subfigure}
    \caption{Numerical simulations of the theoretical framework using the analytical forms of accuracy and agreement. Each plot in the left three columns ablate a single parameters in the framework. The right column shows the effect of coupling two parameters, namely $(t_r, t_d)$ and $(n_r, n_d)$. Changing $t_r$ and $n_r$ alone deviates from GDE, but if they are coupled with dominant features, we can recover GDE (approximately).}
    \label{fig:numerical}
    \vspace{-5mm}
\end{figure*}

We now study the properties of the analytical forms of the expected agreement and the expected accuracy. Instead of bounding their difference, we will use numerical simulation to characterize their properties and difference. The model has $6$ free parameters, namely, $p_d, c, t_d, t_r, n_d, n_r$. We first pick a set of initial values and then vary each values to study the behavior of the model. Unless specified otherwise, the initial values used for all simulations are $p_d=0.7, c=20, t_d=20, t_r=180, n_d=5, n_r=10$. Further, we pick $\zeta(k, c) = 0.9\,\mathbbm{1}\{k > 0\}$. This reflects the intuition that if two models share any features, then with high probability they would agree with each other. This is reasonable if we assume all the models in the same hypothesis distribution are naturally more inclined to agree with each other (\hypertarget{obs4}{\hyperlink{obs4}{O.4}} and Figure~\ref{fig:similarity_vs_error} show that for a \textit{10-class} classification the shared error is at least 35\%). We study the properties and effects of $\zeta$ in Appendix~\ref{app:diff_zeta}.

In the left 3 columns of Figure~\ref{fig:numerical}, we vary each parameter of the framework over a wide range of values. We observe that for both $p_d$ and $c$, the agreement closely track each other for a large portion of the parameter values. This suggests that the difference between generalization error and agreement is robust to how much of the data have dominant features and the size of the model. Further, we observe both accuracy and agreement saturate as the model capacity, $c$, increases. This is equivalent to increasing the model capacity with infinite amount of training data. This is consistent with prior works on \textit{model scaling}~\citep{tan2019efficientnet} which suggests that model size may be related to how many features the model can learn. On the other hand, the behaviors of agreement and accuracy appear to be more sensitive to the other parameters that describe the relationship between total numbers of existing features and how often these features appear in a single data point, in particular $t_r$ and $n_r$, quantities that govern the distribution of rare data. Intuitively, the rare features and data represent the part of data distribution that appear in the tail of the data distribution, and require \textit{memorization} to learn~\citep{feldman2020does}.

The observations about $n_r$ and $t_r$ suggest that GDE requires some distributional assumptions on the features and data in our framework (and in reality~\citep{jiang2022assessing}). One possible hypothesis is that the relationship between $t_r$ and $t_d$ and the relationship between $n_r$ and $n_d$ follow the Pareto principle~\citep{pareto1964cours} (given the long-tailed behavior observed in \hyperlink{obs1}{O.1}). To verify the effect of this hypothesis, we vary $n_r$ and $t_r$ while keeping $n_d$ and $n_r$ proportional to them, that is, $n_d = \lfloor\alpha n_r\rfloor$ and $t_d = \lfloor\alpha t_r\rfloor$. We choose $\alpha = 0.2$ and show the results the in right column of Figure~\ref{fig:numerical}. Notice that if the ratio between these quantities is constant, agreement once again tracks the accuracy closely, indicating that the relationship between dominant and rare  data is central to the origin of GDE in this model.



==> sec_theory.tex <==
\section{A Combinatorial Framework of Feature Learning}
\label{sec:toy_model}

In this section, we present a new framework of feature learning for a binary classification\footnote{This can be extended to multi-class without significant modification.} based on the insights from the experiments above. We saw in \hyperlink{obs1}{O.1} that the distribution of features is long-tailed. This means a relative small number of unique features constitute a large proportion of all the features that appear in the data. To facilitate analysis, we will assume there are two types of features, \textit{dominant features} and \textit{rare features}, where the dominant features appear with much higher probability than rare features. Further, we observed that data with high confidence tend to have much fewer features than the ones with high confidence (\hyperlink{obs2}{O.2}). To model this behavior, we will assume that there are two types of data points: \textit{dominant data} and \textit{rare data}. The former contains a small number of dominant features and the later contains a larger number of rare features. This is another simplification based on \hyperlink{obs2}{O.2}, which shows that high-confidence data tend to have fewer high-frequency features.

\paragraph{Definitions and additional notations.} Before describing the full model, we first define the parameters of the model as well as some additional notations:
\begin{itemize}
    \item $p_d$: the proportion of all data that are dominant.
    \item $p_r$: the proportion of all data that are rare. This parameter is equal to $1-p_d$.
    \item $c$: the total model capacity. It represents how many features a single model can learn.
     \item $t_d$: the total number of dominant features available in the data for one class.
    \item $t_r$: the total number of rare features available in the data for one class.
    \item $n_d$: the total number of dominant features a single dominant data point has. $n_d \leq t_d$.
    \item $n_r$: the total number of rare features a single rare data point has. $n_r \leq t_r$.
\end{itemize}
We will use $\Pi(\cdot)$ to denote the set of all features a model or a feature have.

\paragraph{Data generating process.} We can see the data generating process as the following sampling procedure. First, we decide which class the data point belongs to. We are considering a class balanced binary classification problem so each class occurs with equal probability of $\frac{1}{2}$. Then, we decide whether the data point is dominant or rare. This is the equivalent to sampling from a Bernoulli distribution, $\text{Ber}(p_d)$. If the data point is dominant, we sample $n_d$ dominant features uniformly \textit{without} replacement. Vice versa, if the data point is rare, we sample $n_r$ dominant features uniformly \textit{without} replacement. It is easy to verify that the proportion of dominant data points and features is $p_d$ and the proportion of rare data points and features is $p_r$.

\paragraph{How the models learn.} We saw in \hyperlink{obs3}{O.3} that the frequency of features occurring in different models is positively correlated with the frequency at which the features occur in the data. We can model the learning process as another \textit{sampling-without-replacement} process where the probability that a model learns a feature is \textit{proportional} to the frequency at which the feature occurs in the data. Under this assumption, in expectation, $c_d = \frac{1}{2} p_d  c$ of the features in a single model would be dominant features for a single class, and $c_r = \frac{1}{2} p_r  c$ of the features for a single class would be rare. We can further simplify this process by assuming that the model will always sample $c_d$ dominant features for each class, and $c_r$ rare features for each class\footnote{Both $c_r$ and $c_d$ are rounded to the nearest integer such that the total number of features in a model is still $c$.}.

\paragraph{How the models make predictions.} For a data point $x$ and a model $f$, we assume that the model will correctly classify $x$ if the overlap between the features of $x$ and the features of $f$ is not empty. Otherwise, the model will perform a random guess. The expected error that a single model $f$ makes on a single datum pair $(x,y)$ is thus $\msf{err}(f, x, y) = \frac{1}{2}\mathbbm{1}\left\{\Pi(f) \cap \Pi(x) = \varnothing \right\}$.
Further, given a pair of models $(f,g)$ and a single datum pair $(x,y)$, there are three distinct behaviors for how they will make predictions. \textbf{(1)} The two models will always agree with each other if both of them share feature with $x$, since both will classify $x$ correctly (i.e., if $|\Pi(f) \cap \Pi(x)| > 0$ and $|\Pi(g) \cap \Pi(x)| > 0$). \textbf{(2)} If the models both do not share any features with $x$, then by the previous assumptions, the models will make random guesses; however, if the models share features with each other, their random guesses will not be independent from each other (\hyperlink{obs4}{O.4}). We hypothesize that how two models agree with each other is a function of $k$, the number of features they share, and $c$, the model capacity. We capture this intuition with an \textit{agreement function},  $\zeta: \sN \times \sN \rightarrow [0, 1]$, which returns the probability that two models will agree based on how many features they share relative to the full model capacity. This function is crucial for understanding how models make mistakes. \textbf{(3)} Finally, if the models do not share any features with each other or with $x$, both models will perform independent random guesses, in which case they will agree $50\%$ of the time.

\paragraph{Remarks.} An important difference between this model and the multi-view model from~\citet{allen2020towards} is that our model does not treat all features as equal. Indeed, the experiments in Section~\ref{sec:exp} show that features demonstrate a wide range behaviors in terms of how often they occur in the data and how they interact with the models. Another notable difference is that in~\citet{allen2020towards}, the multi-view portion of the dataset -- which intuitively are easier to classify -- contains \textit{all} the features in the data. In reality, the ``easy'' part of the data that a large portion of the models classify correctly actually contain much fewer features. These observations suggest that having different types of features is perhaps a more accurate description of nature. Nonetheless, we do not describe the exact mechanism of how feature learning actually happens under our model since we are not assuming any particular hypothesis class. The spirit of our model of feature learning is close to that of~\citet{allen2020towards} and we believe a similar iterative analysis can be applied to our model.

It is also natural to question whether the simplification where a single feature is sufficient for determining the class is sensible. Indeed, in practice, a classifier likely uses more than one feature to determine the correct class. We believe that this simplification is realistic as we are considering a binary classification problem in this framework, and that allowing more features to participate in determining the true class makes the model more expressive but should not fundamentally alter the behavior of the system.
Further, the true distributions of features and data are evidently more complex --- dominant data can contain rare features, and, vice versa, rare data can also contain some dominant features. In fact, the dichotomy may no longer be appropriate as the distribution of features and data becomes more complicated --- both features and data can lie on a continuous spectrum between ``dominant'' and ``rare'' (Figure~\ref{fig:feat_freq} and \ref{fig:conf_feat}). These changes can be smoothly incorporated into the framework by modifying the distribution of features but doing so can increase the complexity of the analysis. An exact analytical solution may become unattainable, but we could leverage tail bounds to characterize the system, a promising direction for future works. Still, we will see that this relatively simplified model readily offers interesting insights into observed phenomena. 

\subsection{Analytical Forms of Accuracy and Agreement}
Using this model, the analytical form of expected accuracy, $\msf{Acc}$, and expected agreement rates, $\msf{Agr}$, can be derived through combinatorics.  All propositions are proven in Appendix~\ref{app:proof}, but the chief point here is that these are both computable in closed form.

\begin{proposition}
Under the model defined above, the expected accuracy over the model distribution and data distribution is:
\begin{align}\label{eqn:acc}
    \msf{Acc} = p_d\left( 1- \frac{1}{2}\frac{{t_d-c_d \choose n_d}}{{t_d \choose n_d}} \right) + p_r\left( 1- \frac{1}{2}\frac{{t_r-c_r \choose n_r}}{{t_r \choose n_r}} \right).
\end{align}
\end{proposition}

\begin{proposition}
For the model above, let ${n \choose r}=0$ when $n < 0$, $r < 0$ or $n < r$,
and let:
\begingroup
\allowdisplaybreaks
\begin{small}
\begin{align*}
    q_1 &= p_d \left(1-\frac{{t_h-c_d \choose n_d}}{{t_d \choose n_d}}\right)^2 + p_r \left(1-\frac{{t_r-c_r \choose n_r}}{{t_r \choose n_r}}\right)^2,   \\
    q_2(k) &= p_d \frac{{t_d-n_d \choose c_d}^2}{{t_d \choose c_d}^2} \left( \sum_{a+b=k} \frac{{c_d \choose a}{t_d-n_d-c_d \choose c_d - a}}{{t_d-n_d \choose c_d}} \frac{{c_r \choose b}{t_r-c_r \choose c_r - b}}{{t_r \choose c_r}} \right) \\
    & \,\,\,\, + p_r \frac{{t_r-n_r \choose c_r}^2}{{t_r \choose c_r}^2} \left( \sum_{a+b=k} \frac{{c_d \choose a}{t_d-c_d \choose c_d - a}}{{t_d \choose c_d}} \frac{{c_r \choose b}{t_r-n_r-c_r \choose c_r - b}}{{t_r-n_r \choose c_r}} \right),
\end{align*}
\end{small}
\endgroup
then the expected agreement between an i.i.d pair of models $(f,g)$ drawn for the model distribution is:
\begin{align}\label{eqn:agr}
    \msf{Agr} = \frac{1}{2} + \frac{1}{2}q_1 + \sum_{k=1}^c \left (\zeta(k, c) - \frac{1}{2} \right) q_2(k).
\end{align}

\end{proposition}

Further, we discuss the origin of irreducible \textit{generalization error} and other properties of this framework in Appendix~\ref{app:error} and show a potential connection between feature learning and data scaling~\citep{hestness2017deep}.

\subsection{Numerical Simulation}

\begin{figure*}[h]
     \centering
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/p_d.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/t_d.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/t_r.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/t_r_t_d.pdf}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/c.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/n_d.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/n_r.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.17\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/n_r_n_d.pdf}
    \end{subfigure}
    \caption{Numerical simulations of the theoretical framework using the analytical forms of accuracy and agreement. Each plot in the left three columns ablate a single parameters in the framework. The right column shows the effect of coupling two parameters, namely $(t_r, t_d)$ and $(n_r, n_d)$. Changing $t_r$ and $n_r$ alone deviates from GDE, but if they are coupled with dominant features, we can recover GDE (approximately).}
    \label{fig:numerical}
    \vspace{-5mm}
\end{figure*}

We now study the properties of the analytical forms of the expected agreement and the expected accuracy. Instead of bounding their difference, we will use numerical simulation to characterize their properties and difference. The model has $6$ free parameters, namely, $p_d, c, t_d, t_r, n_d, n_r$. We first pick a set of initial values and then vary each values to study the behavior of the model. Unless specified otherwise, the initial values used for all simulations are $p_d=0.7, c=20, t_d=20, t_r=180, n_d=5, n_r=10$. Further, we pick $\zeta(k, c) = 0.9\,\mathbbm{1}\{k > 0\}$. This reflects the intuition that if two models share any features, then with high probability they would agree with each other. This is reasonable if we assume all the models in the same hypothesis distribution are naturally more inclined to agree with each other (\hypertarget{obs4}{\hyperlink{obs4}{O.4}} and Figure~\ref{fig:similarity_vs_error} show that for a \textit{10-class} classification the shared error is at least 35\%). We study the properties and effects of $\zeta$ in Appendix~\ref{app:diff_zeta}.

In the left 3 columns of Figure~\ref{fig:numerical}, we vary each parameter of the framework over a wide range of values. We observe that for both $p_d$ and $c$, the agreement closely track each other for a large portion of the parameter values. This suggests that the difference between generalization error and agreement is robust to how much of the data have dominant features and the size of the model. Further, we observe both accuracy and agreement saturate as the model capacity, $c$, increases. This is equivalent to increasing the model capacity with infinite amount of training data. This is consistent with prior works on \textit{model scaling}~\citep{tan2019efficientnet} which suggests that model size may be related to how many features the model can learn. On the other hand, the behaviors of agreement and accuracy appear to be more sensitive to the other parameters that describe the relationship between total numbers of existing features and how often these features appear in a single data point, in particular $t_r$ and $n_r$, quantities that govern the distribution of rare data. Intuitively, the rare features and data represent the part of data distribution that appear in the tail of the data distribution, and require \textit{memorization} to learn~\citep{feldman2020does}.

The observations about $n_r$ and $t_r$ suggest that GDE requires some distributional assumptions on the features and data in our framework (and in reality~\citep{jiang2022assessing}). One possible hypothesis is that the relationship between $t_r$ and $t_d$ and the relationship between $n_r$ and $n_d$ follow the Pareto principle~\citep{pareto1964cours} (given the long-tailed behavior observed in \hyperlink{obs1}{O.1}). To verify the effect of this hypothesis, we vary $n_r$ and $t_r$ while keeping $n_d$ and $n_r$ proportional to them, that is, $n_d = \lfloor\alpha n_r\rfloor$ and $t_d = \lfloor\alpha t_r\rfloor$. We choose $\alpha = 0.2$ and show the results the in right column of Figure~\ref{fig:numerical}. Notice that if the ratio between these quantities is constant, agreement once again tracks the accuracy closely, indicating that the relationship between dominant and rare  data is central to the origin of GDE in this model.


